Non-local quark models for description of dense matter in the cores of neutron stars

This thesis work focuses on studying the possible existence of phase transitions in the immediate compact remnants of core collapse supernova, neutron stars, and the theoretical models that describe the interior of dense matter. Specifically, we are interested in analyzing the feasibility of a transition from hadronic matter to quark matter in the cores of these objects. For the phase transition we will use two different formalisms: the Maxwell formalism or abrupt phase transition and the Gibbs formalisms or mixed phase transition. For the description of hadronic matter, we will use different parametrizations of the relativistic mean field model with density-dependent coupling constants. For the description of quark matter we will use an effective nonlocal Nambu Jona-Lasinio model of three flavors with vector interactions, in which we will include the possibility of formation of diquarks to model a superconducting phase of color in $SU(3)$. Phase diagrams and equations of state of quark matter at finite temperature are presented, and the influence of that type of matter on observables associated with neutron stars is investigated. The simplified thermal evolution of compact stars during their formation is studied, from their state of proto-neutron stars to that of cold neutron stars, and the results obtained are compared with recent astrophysical observations. The results obtained indicate that the occurrence of quark matter in the nuclei of these stars remains a promising possibility. The fact that the use of more realistic models for the description of the dense matter in these objects indicates the presence of quark matter inside neutron stars, could be an answer to the question of the behavior of that kind of matter and the determination of its corresponding equation of state.

==> Resultados/Resultados..bak.tex <==
\chapter{\label{ch:Resultados}Estrellas de neutrones con materia de quarks: resultados}

\section{Aplicación de los modelos a proto-estrellas de neutrones y estrella de neutrones frías}

hasta aquí hemos desarrollado todos los componentes necesarios para modelar el contenido de las estrellas de neutrones. Tenemos por un lado los modelos hadrónicos y de quarks, que nos dan las ecuaciones de estado correspondientes, y en el primer capítulo desarrollamos las ecuaciones dee structura que, ingresando una ecuación de estado, nos permiten obtener la masa, el radio y la masa bariónica de las estrellas. Veamos entonces qué criterios utilizamos para construir las ecuaciones de estado híbridas.  En principio, la trancisión de materia hadrónica a materia de quarks puede ser tanto abrupta (tipo Maxwell), o suave (tipo Gibbs), dependiendo de la tensión superficial entre la interface de quarks y hadrones. En este punto nos encontramos con un problema respecto de qué transición usar, ya que el valor de la tensión superficial es poco conocido. Por ejemplo, los cálculo de lattice QCD predicen un valor que va desde $0$ $MeV/fm^2$ hasta $100$ $MeV/fm^2$ \cite{KAJANTIE1991693}. De acuerdo a estudios teóricos, una tensión superficial del orden de $70$ $MeV/fm^2$ favorecería una transición tipo Maxwell antes que una tipo Gibbs \cite{sotani2011,Yasutake2014}, pero justamente por el alto error al determinar el valor, no podemos en principio elegir un tipo de transición determinada. Dado este problema, es necesario calcular los dos tipos de transición. A la vez, como nos interesa calcular estadíos tempranos de las estrellas, también necesitamos definir que temperatura o entropía deberán tener nuestras ecuaciones de estado, y que fracción leptónica. En lo que sigue, utilizaremos el siguiente criterio: construiremos transiciones de fase a lo Maxwell para distintos valores de interacción vectorial de quarks, y para las parametrizaciones DD2 y GM1L de el modelo hadrónico, todos a temperatura cero. Bajo la restricción de 2 $M_{\odot}$ de las mediciones PSR J1614-2230 and PSR J0348+0432 \cite{Demorest:2010bx,Lynch:2012vv,Antoniadis:2013pzd,Arzoumanian:2017puf}, y la suposición de que las materia de quarks existe en estrellas de neutrones, calculamos la masa máxima de las estrellas para distintos parámetros de interacción vectorial. Esto nos lleva a $0.331<\mathrm{\zeta_v}<0.371$ para GM1L, y
$0.328<\mathrm{\zeta_v}<0.385$ para DD2. El límite inferior se establece en la interacción vectorial mínima necesaria para llegar al límite de $2M_{\odot}$, y el límite superior los definimos al encontrar la interacción vectorial máxima para la cual existe materia de quarks dentro de la estrella. Es decir, interacciones vectoriales superiorres resultan en estrellas puramente de materia hadrónica. Una vez fijadas esas interacciones vectoriales, calcularemos distintas ecuaciones de estado a temperatura y/o entropia fijas y analizaremos distintos estadíos de las estrellas. Luego, realizaremos el mismo análisis con esas interacciones vectoriales fijadas, pero realizando una transición de fase a lo Gibbs.


\subsection{Construcción a lo Maxwell}

Para la construcción a lo Maxwell, buscamos el cruce de la Energía de Gibbs versus la presión para las curvas de hadrones y de quarks como explicamos en la sección \ref{construcciones}. Los cruces para las curvas correspondientes a las interacciones vectoriales mencionadas se muestran en la figura \ref{EoS_maxwell_DD2_GM1L}. En esa figura, se ve que hay dos transiciones visibles. La primera de materia de quarks a materia hadrónica a presión  $P \sim 100 -150$ MeV/fm$^3$, y la segunda a de materia hadrónica a materia de quarks a $P \sim 350 - 400$ ~ MeV/fm$^3$. Las EdE son bastante similares y resulta difícil distinguir entre las dos fases en el rango de las presiones  $P \sim 100 - 400$ MeV/fm$^3$. Esto puede ser interpretado como un comportamiento de enmascaramiento, distinto al de deconfinamiento a materia de quarks pura \cite{Alford:2004pf}. 
     
\begin{figure}[ht!]
\begin{center}
\subfigure{\includegraphics[width=0.45\textwidth]{dd2_eos.pdf}}
\hspace{0.02\textwidth}
\subfigure{\includegraphics[width=0.45\textwidth]{gm1l_eos.pdf}}
\caption[Construcción de EdEs híbridas a lo Maxwell para las parametrizaciones elegidas.]{Izquierda: el panel (a) muestra la construcción de la ecuación de estado (a $T = 0$) de la energía de gibbs por barión $(G)$ para una parametrización híbrida DD2-3nPNJL. La linea negra corresponde la EdE de la parte hadrónica y las lineas punteadas rojas y azules son las EdE para la fase de quarks para los dos valores de interacciones vectoriales. El panel (b) muestra la densidad de energía en función de la presión, para los valores mencionados. Derecha: lo mismo que el panel izquierdo pero para la parametrización híbrida GM1L-3nPNJL.}
\label{EoS_maxwell_DD2_GM1L}
\end{center}
\end{figure}

Puede verse en la figura \ref{masses_gibbs}, que una trransición de fase de primer orden ocurre a $\mu_B \sim$ 940 MeV,indicada por una discontinudad en la densidad de partículas y las masas dinámicas. Esto corresponde a la región donde se termina de desacoplar el quark $s$, como vimos en la sección \ref{const_diag_fases}. Para potenciales químicos entre 940 MeV y 1300 MeV tenemos una fase donde el condensado quiral de los quarks $u$ y $d$ $\langle \bar u\, u\rangle\, =\, \langle \bar d\,d\rangle \,\sim \,0$,  mientras que  $\langle \bar s\,s\rangle \neq 0$. Esa fase tiene una estructura similar a la materia hadrónica y la primera transición de quark a hadrones es no-física, con condensados de quark $s$. Este comportamiento podría indicar la existencia de una fase que tiene aspectos tanto de materia nuclear como materia de quarks (ver \cite{McLerran:2007qj, Baym:2017whm} y las referencias allí mencionadas). A potenciales mayores que $\mu_B$ $\sim 1300$ MeV y presiones P $\sim 135$ $\mathrm{MeV/fm^3}$, el quark $s$ se deconfina, y la EdE corresponde a materia pura de quarks libres, que es la parte que usaremos para construir la EdE híbrida.

\begin{figure}[ht!]
\begin{center}
\includegraphics[width=0.49\textwidth]{mass_dens.pdf}
\caption[Masas dinámicas $M_i$ y densidades $n_i$ de los quarks $u,d,s$ en función del potencial químico bariónico]{Masas dinámicas $M_i$ y densidades $n_i$ de los quarks $u,d,s$ en función del potencial químico bariónico. $n_e$ corresponde a la densidad de electrones. }
  \label{masses_gibbs}
\end{center}
\end{figure}

Una vez que se construye la EdE híbrida, resolvemos las ecuaciones de TOV para encontrar las curvas masa - radio, y  masa -densidad de energía. Esta última curva tiene una función importante en el análisis: comparandola con los valores de la EdE híbrida, es posible identificar a partir de qué valor de densidad de energía estamos en el sector de quarks puros. Identificando ese punto, luego podemos ver en la curva masa-radio a partir de que valores las estrellas se comportan como estrellas híbridas. Los resultados para temperatura cero de este análisis, para las parametrizaciones mencionadas, y sumando la construcción para la EdE con superconductividad de color (2SC) a $T = 0$ se muestran en la figura \ref{masas_radios_T0}. En todos los análisis que siguen nos mantendremos en el límite inferior de las interacciones vectoriales encontradas, ya que es donde mayor cantidad de materia de quarks encontraremos en las estrellas calculadas.


\begin{figure}[ht!]
\begin{center}
\subfigure{\includegraphics[scale = 0.65]{mr_me_T0.pdf}}
\hspace{0.02\textwidth}
\subfigure{\includegraphics[scale = 0.3]{mr_me_T0_2SC.pdf}}
\caption[Masa gravitacional en función del radio y la densidad de energía con EdEs híbridas con y sin superconductividad de color.]{Izquierda: Curvas de masa gravitacional en función de energía y del radio estelar para las parametrizacionies a $T=0$ sin superconductividad de color. Derecha: las mismas curvas que el panel izquierdo pero con la EdE híbrida incluyendo superconductividad de color.}
\label{masas_radios_T0}
\end{center}
\end{figure}


Se puede ver que todas las curvas cumplen el requerimiento de llegar a las dos masas solares. También se puede apreciar que las parametrizaciones con la rama hadrónica correspondiente a DD2 tienen una rama más grande de estrellas híbridas que las parametrizaciones con GM1L. Esto es así porque la EdE hadrónica  DD2 es mas dura que la GM1L en términos de la energía libre de Gibbs, por lo que la transición a materia de quarks ocurre antes. También vemos que en el caso de la EdE con superconductividad de color, primero se da una transición a materia de quarks sin superconductividad, para luego entrar en la fase superconductora. En la tabla \ref{tabla_MR_MB} se ven los resultados para las masas máximas obtenidas en cada caso, donde se aprecia que el hecho de incluir superconductividad baja ligeramente la masa máxima obtenida. Por otro lado, es necesario mencionar que es posible encontrar otras parametrizaciones que cumplan requerimientos de dos masas solares. Como se ve en la figura \ref{Gv04Maxwell}, por ejemplo, si se aumenta la interacción vectorial, se retrasa el inicio de aparición de un nñúcleo de quarks, pero si al mismo tiempo se aumenta la interacción de diquarks, es posible llegar a dos masas solares y que la materia de quarks este presente mucho antes. Sin embargo, esto reduce ligeramente la masa máxima obtenida. En este trabajo, como mencionamos anteriormente, nos quedaremos con el valor más utilizado en la literatura, de $\zeta_D = G_D/G_V = 0.75$. 

\begin{figure}[ht]
\begin{center}
\includegraphics[scale = 0.4]{Gv04Maxwell.pdf}
\caption[Masa gravitacional $M_G$, en función del radio para la parametrización DD2 y $\zeta_V = 0.4$, con distintos valores de acoplamiento de diquarks.]{Masa gravitacional $M_G$, en función del radio para la parametrización DD2 y $\zeta_V = 0.4$, con distintos valores de acoplamiento de diquarks. }
  \label{Gv04Maxwell}
\end{center}
\end{figure}


\begin{table}[ht!]
\begin{center}
\begin{tabular}{|c|c|c|c|c|}\cline{1-4}
% use packages: color,colortbl
\multicolumn{4}{|c|}{$\mathrm{GM1L}$} \\\hline
& $M_{G}~[M_{\odot}]$ & $M_{B}~[M_{\odot}]$ & $\epsilon_{c}
            ~ [\mathrm{MeV/fm^{3}}]$ \\\hline
$\mathrm{Hadronicas\,\, puras}$ & $2.04$ & $2.42$ & $1194.82$ \\
$\mathrm{\zeta_v} = 0.331$ & $2.00$ & $2.36$ & $1077.02$ \\
$(2SC) \mathrm{\zeta_v} = 0.331$ & $1.95$  & $2.30$ & $1026.53$ \\\hline
\multicolumn{4}{|c|}{$\mathrm{DD2}$} \\\hline
& $M_{G}~ [M_{\odot}]$ & $M_{B}~ [M_{\odot}]$ & $\epsilon_{c}
            ~[\mathrm{MeV/fm^{3}}]$ \\\hline
$\mathrm{Hadronicas\,\, puras}$ & $2.11$ & $2.53$ & $1110.68$ \\
$\mathrm{\zeta_v} = 0.328$ & $2.04$ & $2.43$ & $992.88$ \\
$(2SC)\mathrm{\zeta_v} = 0.328$ & $2.02$ & $2.40$ & $948.00$ \\\hline
\end{tabular}
\caption[Resultados de masa gravitacional y masa bariónica para las transiciones a lo Maxwell]{Masa gravitacional $M_G$, masa bariónica $M_B$, y densidad de energía central $\epsilon_c$ para las estrellas de masa máxima obtenidas para las parametrizaciones a $T = 0$.}
\label{tabla_MR_MB}
\end{center}
\end{table}

\begin{figure}[ht]
\begin{center}
\includegraphics[scale = 0.5]{MR_TEMP.pdf}
\caption[$M_G$ en función del radio para EdEs a temperatura y/o entropía finitas.]{Masa gravitacional $M_G$, en función del radio para estrellas híbridas a diferentes temperaturas $T_\textrm{{trans}}$ para la transición de hadrones a quarks.  $Y_L$ es la fracción leptónica y $Y_{\nu_e}$ la fracción de neutrinos. Las lineas verticales marcan el inicio de la materia de quarks decofinada. Con la excepción de las estrellas sin neutrinos ($Y_{\nu_e}=0$), las de  $T_{\rm trans}=0$ ($T_0$) and $T_{\rm trans}=15$ MeV ($T_{15}$), la transición ocurre en el pico de masa máxima. }
  \label{MR_TEMP}
\end{center}
\end{figure}

Para estudiar las proto estrellas de neutrones, necesitamos extender las ecuaciones de estado a temperatura finita. Se sabe por trabajos anteriores (ver por ejemplo \cite{Pons:1998mm}) que las proto estrellas de neutrones son isoentrópicas y no isotérmicas. Para obtener una EdE isoentrópica para la construcción de Maxwell, primero calculamos las EdEs para la parte hadrónica y de quarks, para una temperatura de transición fija (por ejemplo 15 MeV y 30 MeV). Luego de determinar el punto de cruce de las curvas, extendemos las curvas de cada fase isoentrópicamente para esa temperatura de transición. De esta manera, construimos curvas EdEs isoentrópicas para las parametrizaciones utilizadas a $T = 0$, eligiendo temperaturas representativas de transición $T = 15$ MeV y $T  = 30$ MeV. Dependiendo del estadío de evolución de la estrella, tomamos distintas fracciones de leptones $Y_{\nu_e} \neq 0$), y las fracciones de leptones a considerar son $Y_L = Y_e + Y_{\nu_e} =0.2$ o $0.4.$. Las relaciones de masa radio de las estrellas compuestas por ese tipo de materia se muestran en la figura \ref{MR_TEMP}.

Para los valores máximos de interacciones vectoriales obtenidas anteriormente ($\mathrm{\zeta_v} = 0.371$ y $\mathrm{\zeta_v} = 0.385$) encontramos que un incremento en la temperatura (con o sin neutrinos) cancela la formación de materia de quarks en el interior de las estrellas. Las únicas estrellas con materia de quarks para esos valores de interacción vectorial, son las estrellas de temperatura cero. Para el caso de las interacciones vectoriales mínimas, algo parecido sucede. Las diferencias vienen principalmente de si existen neutrinos atrapados en su interior o no. Para la parametrización DD2, por ejemplo, se puede construir una EdE con neutrinos atrapados hasta temperaturas de transición $T_\textrm{{trans}} = 30$ MeV que contengan materia de quarks en su interior. Sin embargo, para la parametrización GM1L, los neutrinos están presentes únicamente hasta $T_\textrm{{trans}} = 15$ MeV, y para temperaturas mayores la estrella se vuelve inestable antes de que la transición hadrones-quarks ocurra.
Como era esperado, en la figura \ref{MR_TEMP} se observa que la influencia de los neutrinos aumenta la masa máxima de la estrella. Esta influencia depende sensiblemente de la composición de la materia (ver \cite{Prakash97} por ejemplo). Si se tienen en cuenta hadrones pesados (como hyperones o resonancias $\Delta$) y quarks, resulta un incremento en la masa máxima. Esto es exactamente lo opuesto a la situacion de las EdEs idealizadas, donde solo se tienen en cuenta nucleones y leptones, y ningún otro componente que ablande la EdE, en cuyo caso el efecto de los neutrinos es reducir la masa máxima.

Hasta ahora calculamos las relaciones de masa radio para distintas ecuaciones de estado que corresponderían a distintos estadíos de las estrellas de neutrones. Sin embargo, por más que aparezca materia de quarks en esos estadíos, eso no quiere decir que sean realmente estadíos previos de las estrellas calculadas a $T = 0$. Para esto tenemos que analizar el diagrama masa gravitacional - masa bariónica. En la figura \ref{MGvsMB} mostramos estas relaciones para los estadíos calculados anteriormente. Asumiendo que estamos trabajando con estrellas aisladas (sin posibilidad de acretar materia), la masa bariónica debe ser una constante durante la evolución de la estrella, esta condición es mostrada con una línea vertical en la figura mencionada. Las barras verticales marcan el inicio de la materia de quarks deconfinada en el núcleo de las estrellas. Las proto estrellas en sus etapas iniciales de evolución (por ejemplo , $s=1$, $Y_L=0.4$ y $s=2$,$Y_L=0.2$) resultan ser estrellas puramente hadrónicas no importa cuán masivas sean. Una vez que se deleptonizan ($Y_{\nu_e}=0$), y sus entropías bajan al orden de $s=1.5$ y $s=0.8$, la densidad a la cual la materia de quarks aparece es alcanzada. Sin embargo, esto sucede en nuestros ejemplos solo para las estrellas que se encuentran en las regiones rgavitacionalmente inestables, donde las prot-estrellas tienen masas bariónicas mayores que la correspondiente masa de la estrella fría. La situación cambia únicamente cuando las estrellas se convierten en estrellas frías ($s=0$, $Y_{\nu_e}=0$), las cuales contienen materia de quarks pura en sus núcleos. En las tablas \ref{mass-radius} y \ref{mass-radius2} mostramos las composiciones de los núcleos de las proto-estrellas según van evolucionando hacia la estrella de masa máxima fría asociada.

\begin{figure}[ht!]
\begin{center}
\includegraphics[width=0.6\textwidth]{MGvsMB.pdf}
\caption[$M_G$ en función de $M_B$ para estadíos de proto-estrellas de neutrones.]{Masa gravitacional versus masa bariónica para los estadíos seleccionados en la evolución de las proto-estrellas de neutrones. Cada línea termina en la estrella de masa máxima de cada estadío. Las líneas verticales indican el inicio de la materia de quarks deconfinada. Las estrellas en la región sombreada son gravitacionalmente inestables.}
\label{MGvsMB}
\end{center}
\end{figure}

\begin{table}[ht!]
{%
\begin{center}
\begin{tabular}{|l|c|c|l|}\cline{1-4}
% use packages: color,colortbl
\multicolumn{4}{|c|}{GM1L y $\mathrm{\zeta_v} = 0.331$} \\ \hline
\multicolumn{1}{|c|}{Estadios} & $M_G~ [M_{\odot}]$ & $R~ {\rm [km]}$
& {Composicion del nucleo}
\\ \hline
$s=1.0\,, ~Y_L = 0.4$ & $2.05$ & $12.75$  &Hadronica pura\\
$s=2.0\,, ~Y_L = 0.2$ & $2.04$ & $12.84$  &Hadronica pura\\
$s=1.5\,, ~Y_{\nu_e} = 0$  & $2.02$ & $ 11.94 $ &Hadronica pura \\
$s=0.8\,, ~Y_{\nu_e} = 0$  & $2.01$ & $ 11.97 $ &Hadronica pura \\
$s~\,=0.0\,, ~Y_{\nu_e} = 0$  & $2.00$ & $11.90$   &Hibrida\\ \hline
\end{tabular}
\caption[Masa, radio y composición del núcleo para las (proto-) estrellas de neutrones con masa bariónica conservada $M_B = 2.36 M_{\odot}$ para la parametrización GM1L.]{Masa, radio y composición del núcleo para las (proto-) estrellas de neutrones con masa bariónica conservada $M_B = 2.36 M_{\odot}$ para la parametrización GM1L.}
\label{mass-radius}
\end{center}
}
\end{table}

\begin{table}[ht!]
{%
\begin{center}
\begin{tabular}{|l|c|c|l|}\cline{1-4}
% use packages: color,colortbl
\multicolumn{4}{|c|}{DD2 y $\mathrm{\zeta_v} = 0.328$} \\ \hline
\multicolumn{1}{|c|}{Estadios} & $M_G ~[M_{\odot}]$ & $R~ {\rm [km]} $
&{Composicion del nucleo}
\\ \hline
$s=1.0\,, ~Y_L = 0.4$ & $2.10$ & $13.09$ &Hadronica pura \\
$s=2.0\,, ~Y_L = 0.2$ & $2.09$ & $13.15$ &Hadronica pura \\
$s=1.5\,, ~Y_{\nu_e} = 0$  & $2.07$ & $ 12.37 $ &Hadronica pura \\
$s=0.8\,, ~Y_{\nu_e} = 0$  & $2.05$ & $ 12.49 $ &Hadronica pura \\
$s~\,=0.0\,, ~Y_{\nu_e} = 0$  & $2.04$ & $12.27$  &Hibrida\\ \hline
\end{tabular}
\caption{Masa, radio y composición del núcleo para las (proto-) estrellas de neutrones con masa bariónica conservada $M_B = 2.43 M_{\odot}$ para la parametrización DD2.}
\label{mass-radius2}
\end{center}
}
\end{table}

Se ha propuesto  \cite{Prakash97,Brown:1993jz} que las proto-estrellas inestables propuestas anteriormente colapsarían en agujeros negros. Mas aún, se mostró en \cite{Prakash97,Vidana:2002rg} que el colapso podría estar relacionado a la presencia de hyperones e isóbaros $\Delta$, y/o materia de quarks, dado que la materia caliente con neutrinos atrapados es capáz de soportar objetos más masivos que las materia estelar fría. Finalmente, para terminar con la construcción de Maxwell, vale destacar que si hubiéramos hecho el mismo proceso con las estrellas frías obtenidas con EdEs híbrida para materia de quarks superconductora de color, hubiéramos llegado prácticamente al mismo resultado, pero con valores de masas máximas ligéramente más pequeños.


\subsection{Construcción a lo Gibbs}

Para analizar la posibilidad de que exista una fase mixta en las estrellas, el tratamiento es tal cual lo explicado en la sección \ref{construcciones}. Por comodidad, repetiremos aqui el sistema de ecuaciones que tiene que cumplirse, a saber

\begin{eqnarray}
 P^H (\mu_B) &=& P^Q(\mu_Q/3) , \\
 T^H (\mu_B) &=& T^Q(\mu_Q/3) , \\
 \epsilon^H (\mu_B) &<& \epsilon^Q(\mu_Q/3) , \\
 E_G^H(\mu_B) &=& E_G^Q(\mu_Q/3) , \\
 \mu_B &=& \mu_Q/3 = (\mu_u+ \mu_d + \mu_s)/3, \\
  Y_L^H (\mu_B) &=& Y_L^Q(\mu_Q/3),
\end{eqnarray}

donde $\{P,T,\epsilon,E_G, Y_L\}$ corresponden a la presión, temperatura, densidad de energía, energía de Gibbs por partícula y densidad leptónica respectivamente. La diferencia fundamental con la construcción a lo Maxwell, radica en que no es posible construir la fase mixta por simple inspección de dónde se cruzan las curvas, si no que hay que crear un código numéricos que contenga ambos códigos (de quarks y hadrones) y que vaya resolviendo cada EdE para cada punto de manera que se cumplan el conjunto de ecuaciones mencionadas. Esto tiene, por un lado la desventaja de que es muy costoso computacionalmente, pero por otro lado la ventaja de que no hay que hacer construcciones isotérmicas primero e isoentrópicas despues. Al estar todo en un mismo código se puede pedir la condición de que la temperatura sea una variable, y que sea igual punto a punto, pidiendo una entropía por barión constante. Los resultados para este tipo de construcciones se muestran en la figura \ref{MGvsMB_Gibbs}

\begin{figure}[ht!]
\begin{center}
\subfigure{\includegraphics[scale = 0.25]{MB_MG_DD2_Gibbs.pdf}}
\hspace{1em}
\subfigure{\includegraphics[scale = 0.25]{MB_MG_GM1L_Gibbs.pdf}}
\caption[$M_G$ en función de $M_B$ para distintos estadíos de estrellas construidas con transición tipo Gibbs.]{Izquierda: Masa gravitacional en función de la masa bariónica para la parametrización DD2 en la construcción de fase mixta, la parte sombreada corresponde a estrellas gravitacionalmente inestables. Las lineas verticales indican el comienzo de la fase mixta, y el asterisco indica el comienzo de la fase pura de quarks . Derecha: las mismas curvas que el panel izquierdo pero con la parametrización GM1L.}
\label{MGvsMB_Gibbs}
\end{center}
\end{figure}

En este tipo de construcción, se pueden observar dos diferencias fundamentales respecto de la construcción a lo Maxwell: primero, se consigue tener materia de quarks en la fase mixta mucho antes que la aparición de materia de quarks pura en la transición abrupta; segundo, un estadío a temperatura no nula ($s = 0.8\, ,\, Y_{\nu_e} = 0$) entra como estadío posible en la evolución, conservando la masa bariónica de la estrella fría. Por otro lado, la parametrización $GM1L$ resulta en una fase mixta más grande que la $DD2$. 

Para completar el análisis, vale preguntarse en qué rangos de temperaturas es que se consigue un estadío previo a las estrellas de neutrones frías. Para eso, mostramoslos perfiles de temperatura para las distintas EdEs estudiadas, los cuales se muestran en la figura \ref{perfilesTemp}.  De analizar la densidad correspondiente a las estrellas que cumplen la conservación de masa bariónica, encontramos que para el estadío ($s = 0.8\, ,\, Y_{\nu_e} = 0$), la temperatura en el centro de la estrella para la parametrización DD2 es $T_{central} \simeq 15$ MeV, y para el caso GM1L,  $T_{central} \simeq 20$ MeV. Por otro lado, del mismo gráfico se puede apreciar claramente que el estadío ($s = 2\, ,\, Y_{\nu_e} = 0.2$) corresponde a la temperatura máxima de las estrellas, siendo hadrónicas puras. Esto es exactamente igual a los resultados obtenidos en el caso a lo Maxwell, lo que nos lleva a pensar dos posibilidades: o bien para coincidir con los resultados de\cite{Prakash:2000jr} donde el estadío de máximo calentamiento corresponde a ($s = 2\, ,\, Y_{\nu_e} = 0.$), hayq ue incluir fenómenos de transporte, o bien que ese cáclulo fue hecho con ecuaciones de estado menos sofisticadas, y el rol de los neutrinos con nuestras EdEs es significantemente distinto como para llegar a máximo calentamiento antes de que los neutrinos se escapen.


\begin{figure}[ht!]
\begin{center}
\subfigure{\includegraphics[scale = 0.25]{temp_profiles_DD2.pdf}}
\hspace{1em}
\subfigure{\includegraphics[scale = 0.25]{temp_profiles_GM1L.pdf}}
\caption[Perfiles de temperatura en función de la densidad bariónica.]{Izquierda: Temperatura en función de la densidad bariónica para las distintas EdEs analizadas, para la parametrización DD2. Los puntos llenos marcan la densidad correspondiente a la densidad central de la estrella de masa máxima para cada curva. Izquierda: lo mismo que el panel derecho pero para la parametrización GM1L.}
\label{perfilesTemp}
\end{center}
\end{figure}


Finalmente, para terminar el análiss de la fase mixta, nos resta ver cuál es el efecto de la superconductividad de color en las estrellas frías. Como era de esperarse, la inclusión de este efecto baja la masa máxima obtenida, al punto que para la parametrización GM1L, no se alcanza la condición de las dos masas solares, como se puede ver en la figura \ref{2sc_mixed_TOV}. Por otro lado, aunque la parametrización DD2 llega a las dos masas solares, baja sensiblemente la masa bariónica obtenida respecto del caso sin superconductividad de color. Como se puede ver en la figura \ref{MB_MG_2sc_dd2}, el incluir superconductividad nos lleva a una estrella fría que no tiene estadíos anteriores de estrellas con materia de quarks pura ni en fase mixta con la materia hadrónica. Este efecto era el esperado al incluir superconductividad, y sería de esperar que incluyendo este efecto a temperatura finita, también baje las masas bariónicas de esos estadíos, y genere que la materia de quarks aparezca antes. Sin embargo, como mencionamos anteriormente, el tratamiento de superconductividad a temperatura finita entra en conflicto con la inclusión del loop de Polyakov, y no se puede hacer el tratamiento de los dos efectos simultáneamente, por lo cual nos quedaremos simplemente con la interpretación de los datos obtenidos a temperatura cero. Por último, los resultados para las masas, radio y composición del núcleo de las estrellas que conservan masa bariónica en la construcción de fase mixta, se muestran en las tablas \ref{mass-radius_gibbs} y \ref{mass-radius_gibbs2} para las parametrizaciones DD2 y GM1L respectivamente.


\begin{figure}[ht!]
\begin{center}
\subfigure{\includegraphics[scale = 0.25]{2sc_mixed_TOV_dd2.pdf}}
\hspace{1em}
\subfigure{\includegraphics[scale = 0.25]{2sc_mixed_TOV_gm1l.pdf}}
\caption[Perfiles de masa-radio para las estrellas híbridas con superconductividad de color.]{Izquierda: Perfiles de masa-radio para las estrellas híbridas con superconductividad de color para la parametrización DD2.  Izquierda: lo mismo que el panel derecho pero para la parametrización GM1L.}
\label{2sc_mixed_TOV}
\end{center}
\end{figure}



\begin{figure}[ht!]
\begin{center}
\includegraphics[width=0.6\textwidth]{MB_MG_2sc_dd2.pdf}
\caption[$M_G$ en función de $M_B$ para estadíos de proto-estrellas y estrella fría con superconductividad de color.]{Masa gravitacional versus masa bariónica para los estadíos seleccionados en la evolución de las proto-estrellas de neutrones, con la estrella fría correspondiente a la EdE con parametrización DD2 y superconductividad de color.}
\label{MB_MG_2sc_dd2}
\end{center}
\end{figure}


\begin{table}[ht!]
{%
\begin{center}
\begin{tabular}{|l|c|c|l|}\cline{1-4}
% use packages: color,colortbl
\multicolumn{4}{|c|}{DD2 y $\mathrm{\zeta_v} = 0.328$} \\ \hline
\multicolumn{1}{|c|}{Estadios} & $M_G~ [M_{\odot}]$ & $R~ {\rm [km]}$
& {Composicion del nucleo}
\\ \hline
$s=1.0\,, ~Y_L = 0.4$ & $2.13$ & $11.88$  &Hadronica pura\\
$s=2.0\,, ~Y_L = 0.2$ & $2.12$ & $11.96$  &Hadronica pura\\
$s=1\,, ~Y_L = 0.05$  & $2.05$ & $ 11.61 $ &Hadronica pura \\
$s=0.8\,, ~Y_{\nu_e} = 0$  & $2.04$ & $ 11.60 $ &Hadronica pura \\
$s~\,=0.0\,, ~Y_{\nu_e} = 0$  & $2.03$ & $11.56$   &Hibrida\\ \hline
\end{tabular}
\caption{Masa, radio y composición del núcleo para las (proto-) estrellas de neutrones con masa bariónica conservada $M_B = 2.42 M_{\odot}$ para la parametrización DD2 y fase mixta de hadrones y quarks.}
\label{mass-radius_gibbs}
\end{center}
}
\end{table}


\begin{table}[ht!]
{%
\begin{center}
\begin{tabular}{|l|c|c|l|}\cline{1-4}
% use packages: color,colortbl
\multicolumn{4}{|c|}{GM1L y $\mathrm{\zeta_v} = 0.331$} \\ \hline
\multicolumn{1}{|c|}{Estadios} & $M_G~ [M_{\odot}]$ & $R~ {\rm [km]}$
& {Composicion del nucleo}
\\ \hline
$s=1.0\,, ~Y_L = 0.4$ & $2.08$ & $13.10$  &Hadronica pura\\
$s=2.0\,, ~Y_L = 0.2$ & $2.06$ & $12.51$  &Hadronica pura\\
$s=1\,, ~Y_L = 0.05$  & $2.02$ & $ 12.01 $ &Hadronica pura \\
$s=0.8\,, ~Y_{\nu_e} = 0$  & $2.01$ & $ 11.95 $ &Hibrida \\
$s~\,=0.0\,, ~Y_{\nu_e} = 0$  & $2.00$ & $11.85$   &Hibrida\\ \hline
\end{tabular}
\caption{Masa, radio y composición del núcleo para las (proto-) estrellas de neutrones con masa bariónica conservada $M_B = 2.36 M_{\odot}$ para la parametrización GM1L y fase mixta de hadrones y quarks.}
\label{mass-radius_gibbs2}
\end{center}
}
\end{table}


